AT1 fourth-order isogeometric phase-field modeling of brittle fracture

A crucial aspect in phase-field modeling, based on the variational formulation of brittle fracture, is the accurate representation of how the fracture surface energy is dissipated during the fracture process in the energy competition within a minimization problem. In general, the family of AT1 functionals showcases a well-defined elastic limit and narrow transition regions before crack onset, as opposed to AT2 models. On the other hand, high-order functionals provide similar accuracy as low-order ones but allow for larger mesh sizes in their discretization, remarkably reducing the computational cost. In this work, we aim to combine both these advantages and propose a novel AT1 fourth-order phase-field model for brittle fracture within an isogeometric framework, which provides a straightforward discretization of the high-order term in the crack surface density functional. For the introduced AT1 functional, we first prove a {\Gamma}-convergence result (in both the continuum and discretized isogeometric setting) based on a careful study of the optimal transition profile, which ultimately provides the explicit correction factor for the toughness and the exact size of the transition region. Fracture irreversibility is modeled by monotonicity of the damage variable and is conveniently enforced using the Projected Successive Over-Relaxation algorithm. Our numerical results indicate that the proposed fourth-order AT1 model is more accurate than the considered lower-order AT1 and AT2 models; this allows to employ larger mesh sizes, entailing a lower computational cost.

==> conclusion.tex <==
% !Tex root=AT1IV.tex


\section*{Conclusion}
In this work, a novel AT1 fourth-order model for phase-field brittle fracture is proposed within an IgA framework that allows us to discretize the high-order differential operator thanks to the high continuity of the IgA shape functions. First of all we assess the elastic limit of this model, which confirms that higher-order formulations, given the higher regularity, anticipate fracture nucleation. Then, we propose a workflow for the the fourth-order AT1 profile derivation. This method has general validity and allows to obtain the profile shape and regularization constant c$_\ww$ for any combination of coefficients of the energy dissipation integral. Considering a set of coefficients $\{a, \,b, \,c\} = \{1, \, 1, \, 1\}$, we observed that the proposed AT1 fourth-order model is more accurate than the classical AT-models present in the literature. Results confirm our findings in \cite{greco2024higher} pointing out that also the proposed AT1 fourth-order formulation shows a comparable accuracy with respect to the second-order one when considering a coarser mesh. As the dissipation functional coefficients considerably influence the shape of the profile, as well as the limit of the interval where the phase-field is positive, we propose to define the mesh size as a function of the \textit{R} parameter obtaining meshes $R$ times larger than the ones obtained considering the classical rule of thumb, i.e.,  four element resolving the internal length parameter. Then, a sensitivity analysis on the dissipation coefficient has been carried out, leading to the observation that, even though there is not a specific set of coefficients providing significantly better results, high values of \textit{\textit{c}} give more regularity to the solution, tend to reduce errors and allow for larger mesh sizes. Consequently, this entails a significant decrease in terms of the number of degrees of freedom of the problem and the overall computation time. Among future works, we will extend current formulation analysed in the context of both 2D problems and Kirchhoff-Love shells to dynamics. We also want to focus on understanding possible different ways of error assessment to free ourselves from fracture length assessment. Furhtermore, we will possibly include in current simulation framework THB-splines adaptivity and multi-patch geometries \cite{bracco2023adaptive}.  
